Node and Edge Differential Privacy for Graph Laplacian Spectra: Mechanisms and Scaling Laws

This paper develops a framework for privatizing the spectrum of the graph Laplacian of an undirected graph using differential privacy. We consider two privacy formulations. The first obfuscates the presence of edges in the graph and the second obfuscates the presence of nodes. We compare these two privacy formulations and show that the privacy formulation that considers edges is better suited to most engineering applications. We use the bounded Laplace mechanism to provide differential privacy to the eigenvalues of a graph Laplacian, and we pay special attention to the algebraic connectivity, which is the Laplacian's second smallest eigenvalue. Analytical bounds are presented on the the accuracy of the mechanisms and on certain graph properties computed with private spectra. A suite of numerical examples confirms the accuracy of private spectra in practice.

==> consensus.tex <==
\section{Applications to Consensus}
\label{sec:consensus}
In this section, we solve Problem~\ref{prb:prob5} and bound the error in consensus convergence rates when they are computed using private values of~$\lambda_2$. 
As discussed in the introduction, consensus protocols underlie a number of multi-agent control and optimization algorithms, e.g.,~\cite{ren07,olfati04,gennaro06,nedic18}. 
Consider a network of~$n$ agents running a consensus protocol with communication topology modeled by an undirected, unweighted graph $G$. 
%Applications of consensus protocols include formation control for autonomous agents, load balancing, and reaching agreement in a blockchain. Here, we consider the scenario where we have a network and we are receiving queries for $\lambda_2$ from third parties that could potentially be adversaries, these queries are used to estimate how fast our network will reach consensus. 
To protect the connections in this graph, a
differentially private version of~$\lambda_2$ is used for analysis. This computation would be performed, for example, by a network analyst who only has access to the private value of $\lambda_2$ that has been shared by a data curator.
%The rest of this section is organized as follows: we provide the necessary background on consensus, we then give a concentration bound on convergence rate estimates when $(\epsilon,\delta)-$differential privacy is implemented, and lastly we give a bound on the time required for the error of a convergence rate estimate to be within some threshold with low probability.

In continuous time, a consensus protocol takes the form $\dot{x}=-L(G)x,$ where $L(G)$ is the graph Laplacian. This protocol converges 
to the average of agents' initial state values with worst-case error bound at time~$t$ proportional to~$e^{-\lambda_2 t}$ \cite{Mesbahi2010}. 
Let $r(t)=e^{-\lambda_2 t}$ be the true convergence rate for the network $G$. 
Let $\tilde{\lambda}_2$ be the output of the bounded Laplace mechanism with privacy parameters $\epsilon$ and $\delta$. 
Let $\tilde{r}(t)=e^{-\tilde{\lambda}_2 t}$ be the corresponding convergence rate estimate. To compare the estimated convergence rate 
under privacy to the true convergence rate, we analyze $|\tilde{r}(t)-r(t)|$. 

Note that as $t\to \infty$, both~$\tilde{r}(t)\to 0$ and $r(t)\to 0$, which implies that $|\tilde{r}(t)-r(t)|\to 0$ as well. 
Although the error in the convergence rate estimate goes to~$0$ asymptotically, we are interested in analyzing the error 
at all values of $t,$ which will give insight into the short-run utility of private convergence rate estimates. 
To accomplish this, we give a concentration bound that bounds the 
probability $\mathbb{P}\left(|\tilde{r}(t)-r(t)|\geq a\right)$ in terms of~$t$, the true algebraic connectivity~$\lambda_2$, and the level of the privacy encoded in $b$ that is determined using $\epsilon$ and $\delta$.

\begin{theorem}[\emph{Convergence rate concentration bound; Solution to Problem 2}] \label{thm:consensus}
Let $C_{\lambda_2}(b)=1-\frac{1}{2}\left(e^{-\frac{\lambda_{2}}{b}}+e^{-\frac{n-\lambda_{2}}{b}}\right)$. 
Then, for $t > 0$ and a fixed $\lambda_{2}$ and $b$,
\begin{equation}
\mathbb{P}\left(|\tilde{r}(t)-r(t)|\geq a\right)\leq \frac{1}{C_{\lambda_2}(b)}\frac{1}{2a}\left(\rho_1(t)+\rho_2(t)-\rho_3(t)\right),
\end{equation}
where
\begin{align}
    \rho_1(t) &= \frac{e^{-\lambda_{2}(\frac{1}{b}+t)}\left(-bte^{\frac{\lambda_{2}}{b}}+bt+e^{\lambda_{2}t}-1\right)}{bt-1}, \\
    \rho_2(t) \!&=\! e^{-\lambda_{2}t}\left(1-e^{\frac{\lambda_{2}-n}{b}}\right)\!, \,\,
    \rho_3(t) \!=\! \frac{e^{-\lambda_{2}t}-e^{\frac{\lambda_{2}-n(bt+1)}{b}}}{bt+1}.
\end{align}
\end{theorem}

\emph{Proof:} See Appendix~\ref{sec:proof_thm_3}.
 \hfill $\blacksquare$

Taking limits of the bound in Theorem~\ref{thm:consensus} shows that as $t\to\infty,$ $\mathbb{P}\left(|\tilde{r}(t)-r(t)|\geq a\right)\to 0$ for all $a$, and thus this bound has the expected asymptotic behavior. 

We can use Theorem~\ref{thm:consensus} to further characterize the transient response of error in the estimated
consensus convergence rate. 
Specifically, we can bound the 
time required for the error in the convergence rate estimate to be 
larger than some threshold~$a$ only with probability smaller than $\eta$. Formally, 
given a threshold~$a > 0$ and probability~$\eta > 0$,
we bound the times~$t$ for which~$\mathbb{P}\left(|\tilde{r}(t)-r(t)|\geq a\right)\leq  \eta$. 

\begin{theorem} \label{thm:times}
Fix $a > 0$ and ${\eta \in (0, 1)}$. 
Let~${\epsilon > 0}$ and~${\delta \in (0, 1)}$ be given and compute the scale parameter~${b > 0}$. 
Consider a graph on~$n$ nodes with algebraic connectivity~$\lambda_2$.
If~$\lambda_2 \leq \frac{n}{2}$, then 
we have~$\mathbb{P}\left(|\tilde{r}(t)-r(t)|\geq a\right)\leq\eta$
for 
\begin{equation}
t\geq\frac{\left(e^{-\frac{\lambda_{2}}{b}}-e^{\frac{\lambda_{2}-n}{b}}\right)\frac{b}{\lambda_{2}e}+2aC_{\lambda_2}(b)\eta+1}{2aC_{\lambda_2}\eta b}. 
\end{equation}
If~$\lambda_{2}>\frac{n}{2}$, then the desired bound holds for~$t\geq\frac{2aC_{\lambda_2}(b)\eta+1}{2aC_{\lambda_2}(b)\eta b}$. 
\end{theorem}
\emph{Proof:} 
%Ideally, we would solve the inequality $\frac{1}{C_{\lambda_2}}\frac{1}{2a}\left(\rho_1(t)+\rho_2(t)-\rho_3(t)\right)\leq \eta$ in terms of $t$, however this does not have a closed form solution. 
See Appendix~\ref{sec:proof_times}.
\hfill $\blacksquare$

We note that the statistics of the differential privacy mechanism can be released
without harming privacy. Therefore, the values of~$C_{\lambda_2}(b)$ and~$b$
can be publicly released. A network analyst can thus compute these bounds
for any choices of~$a$ and~$\eta$ of interest. Because the exact
value of~$\lambda_2$ is unknown, they can compute the maximum
value of these two times to find a time after which the
desired error bound always holds. 


Notice that the two conditions on $t$ in Theorem~\ref{thm:times} 
only vary by a factor of $\left(e^{-\frac{\lambda_{2}}{b}}-e^{\frac{\lambda_{2}-n}{b}}\right)\frac{b}{\lambda_{2}e}$ in the numerator, 
and when $\lambda_2$ is large this term is negative. 
This means that if $\lambda_2$ is large, the required time for~$\mathbb{P}\left(|\tilde{r}(t)-r(t)|\geq a\right)\leq\eta$ is smaller than if $\lambda_2$ was small.

\subsection{Consensus Simulations}
\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{calvin_sim.pdf}
    \vspace{-5mm}
    \caption{The top plot shows $500$ sample convergence rate estimates~$\tilde{r}_i(t)=e^{-\tilde{\lambda}_2^i t}$, where~$\tilde{\lambda}_2^i$ is the output of 
    the~$i^{th}$ trial of the bounded Laplace mechanism with $\epsilon=0.4,\ \delta=0.05,$ and $A=1$ for a network of $n=10$ agents with $\lambda_2=1.$ The set $S(t)$ 
    shown on these plots is defined as~${S(t) = \{\tilde{r}_i(t) : \tilde{r}_i(t) = e^{-\tilde{\lambda}_2^it} \textnormal{ and } |\tilde{r}_i(t)-e^{-\lambda_2t}|\leq a\}}$ with $a=0.2.$ The bottom plot shows the lower bound on $P(\tilde{r}_i(t)\in S)$ obtained by using Theorem~1 in~\eqref{eq:simlowerbound}. 
    This lower bound approaches $1$ relatively quickly and is consistent with the sample convergence rates shown in the top plot.}
    \label{fig:cal_sim}
\end{figure}
Consider a network of $n=10$ agents with $\lambda_2=1$ and a true convergence rate of $r(t)=e^{-\lambda_2 t} = e^{-t}$.  
The network operator wishes to privatize~$\lambda_2$ 
 using the bounded Laplace mechanism with $\epsilon=0.4,\ \delta=0.05,$ and $A=1.$ 
 Solving for $b$ with the algorithm in \cite{holohan2018bounded} yields $b\geq7.39,$ and selecting $b=7.39$ ensures $(0.4,0.05)-$differential privacy. Let $\tilde{\lambda}_2$ 
 be the private output of the bounded Laplace mechanism. 
 Then, for a recipient of~$\tilde{\lambda}_2$, 
 the estimated consensus convergence rate is~$\tilde{r}(t)=e^{-\tilde{\lambda}_2 t}$. 
 Let $P\big(|\tilde{r}(t)-r(t)|\leq a\big)$ be the the probability of the error of the convergence rate estimate being less than $a$ at time $t$. 
 Intuitively, $P\big(|\tilde{r}(t)-r(t)|\leq a\big)$ should be close to $1$ as~$t$ grows. 
 
 %Let $S=\{\tilde{r}(t) :|\tilde{r}(t)-e^{-\lambda_2 t}|\leq a\}.$ Note that $P(\tilde{r}_i(k)\in S)$ changes with time based on the results in Section IV, and 
 We can lower bound~$P\big(|\tilde{r}(t)-r(t)|\leq a\big)$ by noting that 
 \begin{equation} \label{eq:simlowerbound}
 P\big(|\tilde{r}(t)-r(t)|\leq a\big)=1-P\big(|\tilde{r}(t)-r(t)|\geq a\big), 
 \end{equation}
 which we can use Theorem~\ref{thm:consensus} to bound. 
 To that end, 
 Figure~\ref{fig:cal_sim} shows how~$P\big(|\tilde{r}(t)-r(t)|\leq a\big)$ 
 changes with time for $a=0.2$ and shows $500$ sample convergence rate estimates 
 for values of~$\lambda_2$ privatized with the parameters from above.

These simulations show that for a sufficiently large~$t$, $P\big(|\tilde{r}(t)-r(t)|\leq a\big)$ is close to $1$ and that the times $t$ 
for which this occurs are often small. 
This occurs because the bounded Laplace mechanism outputs $\tilde{\lambda}_2 \in [0,n]$,
and thus~$\tilde{r}(t)\to 0$ as $t\to \infty$ for any~$\tilde{\lambda}_2$, while 
the true convergence rate~$r(t)$ also converges to $0$. These results also show that Theorem~1 is consistent with intuition as highlighted in 
Figure~\ref{fig:cal_sim}, namely that as $t$ grows the error in any estimated convergence rate using the output of the bounded Laplace mechanism converges to 0
eventually. 

Beyond the consensus protocol, the value of~$\lambda_2$ is related to many other
graph properties~\cite{abreu07}, and we next show how the private value of~$\lambda_2$
can still be used to accurately bound two other properties of interest. 


